10^(10^6) Worlds and Beyond: Efficient Representation and Processing of Incomplete Information

Current systems and formalisms for representing incomplete information generally suffer from at least one of two weaknesses. Either they are not strong enough for representing results of simple queries, or the handling and processing of the data, e.g. for query evaluation, is intractable. In this paper, we present a decomposition-based approach to addressing this problem. We introduce world-set decompositions (WSDs), a space-efficient formalism for representing any finite set of possible worlds over relational databases. WSDs are therefore a strong representation system for any relational query language. We study the problem of efficiently evaluating relational algebra queries on sets of worlds represented by WSDs. We also evaluate our technique experimentally in a large census data scenario and show that it is both scalable and efficient.

==> futurework.tex <==

\section{Future Work}
\label{sec:future}


While first experiments suggest that WSDs are a very
promising framework for representing and managing incomplete information, we
are currently working on evaluating WSDs in applications other than survey
data.

We have started the analysis of the data cleaning problem in the context of
UWSDTs and our experiments make use of partially cleaned data.
%
%Our main contribution regarding data cleaning was to
%embed it into our framework and to produce realistic
%world-sets beyond or-set relations for our experiments.
%
In the future, we will study the data
cleaning problem within our framework in greater depth.

Although in many application scenarios, e.g. census, the data does not change over time, 
we intend to address the problem of making {\em updates}\/ to WSDs in the future.
Note that updates are easy to handle in the case when changes made are the
same in all worlds. For instance, adding a tuple to each world of a UWSDT
just means to add the tuple once to the template relation. However, updating
world-sets with incomplete information -- even defining meaningful notions of
this -- is an interesting problem for future research.

We plan to generalize the framework of WSDs to support also 
infinite sets of possible worlds by taking an approach that integrates WSDs
with c-tables. Our WSDs correspond to a certain CNF-like {\em normal form}\/
for the condition formulas in c-tables. In the future, we would like to
elaborate on this to define syntactic normal forms for c-tables which are at
the same time powerful as representation systems (for finite as well as
infinite world-sets) and allow for scalable representation, data cleaning, and
query processing.


%%% Local Variables: 
%%% mode: latex
%%% TeX-master: 569
%%% TeX-master: "569"
%%% End: 

